H\"older properties of Weierstrass-like solutions of $\theta$-twisted cohomological equations

It is proved that bounded solutions of modified ($\theta$-twisted) cohomological equations for expanding circle maps are $\theta$-H\"{o}lder continuous but are not $(\theta+\gamma)$-H\"{o}lder continuous for every $\gamma>0$ at almost every point. This gives new examples of "nonlinear" Weierstrass-like functions for which the optimal \holder exponent at most points is known.

==> bound_distort.tex <==
%\begin{lm}[Distortion estimate]  \label{lm:bdistort}
%There exists a contstant $\Cbdistort$
%such that for
%every $x\in\mfd$,
%every natural $N$ and every $h>0$ such that
%\begin{equation}
%    h \leq \frac{1}{\Cbdistort} \frac{1}{\dfxx{N}{x} } < 1
% \label{neq:hcond_bdist} 
%\end{equation}
%for every $\sigma \in \{ -1,1 \} $
%the following estimates hold:
%\begin{equation*}
%    \frac{1}{\Cbdistort} \leq
%    \frac{\dfxx{N}{x}}{\dfxx{N}{x+\sigma h}}
%    \leq \Cbdistort 
%    .
%\end{equation*}
%\end{lm}

\begin{proof}[Proof of Lemma \ref{lm:bdistort} ]
    Fix a natural $N>0$ and $x\in\mfd$.
    %Note that $\mfd = [0,1]$. % / \sim = [x-1/2,x+1/2] / \sim$.
    Let $F:\Rb \to \Rb$ be a lift of $f$.
    Let $J\subset S^1$ be a minimal by inclusion segment containing $x$
    such that
    %$[x,x+h] \subset J$ and 
    $F^N(J) = [0,1]$.
    It implies that $f^N$ is injective (strictly monotone)
    on $J$.
    Changing the lift if necessary (by adding a constant)
    we may assume that $x$ is a center of $J$.

    A standard calculation (see \cite{MANE_ERGTH}, p169) 
    %\cite{LUZZ_BDIST}, Theorem 5, for example)
    shows that
    there exists a constant $C$
    (depending only on $f$) such that
    for every $x_1,x_2\in J$ 
    \begin{equation}
        1/C \leq \frac{\dfxx{i}{x_1}}{\dfxx{i}{x_2}}
        \leq C, \quad 1\leq i \leq N
        \label{neq:bdistort_estim}
    \end{equation}

    We want now to estimate size of $J$.
    Suppose $J = [a,b]$. 
    Then $F^N(b) - F^N(a) = 1$. 

%    [Strictly speaking I can not put $1$ here because $S^1 = [0,1]/\sim$.
%    So I could put something like $1-\omega$ for small $\omega$, it would
%        just alter slightly resulting $C_3$ but it would require me
%    to say more words]

    Thus
    \begin{equation*}
        1 =  F^N(b) - F^N(a) = (F^N)'(\xi) (b-a) = \dfxx{N}{\xi} (b-a)
    \end{equation*}
    for some $a < \xi < b$.

    It follows that 
    \begin{equation*}
        b-a =
        \frac{1}{\dfxx{N}{\xi}} \geq \frac{1}{C}
        \frac{1}{\dfxx{N}{x}}
    \end{equation*}

    Take $\Cbdistort = 2C$. 
    Now for every
    $h$ satisfying the condition \eqref{neq:hcond_bdist}
    we have $x+\sigma h \in J$ for every $\sigma$ from
    $\{ -1,1 \}$.
    Then estimates \eqref{neq:bdistort_estim} hold.
\end{proof}

%\begin{rem}
%    Following \cite{MANE_ERGTH}
%    the constant can be written explicitly
%    \begin{equation*}
%        \Cbdistort = 2\exp \enbrace{ \frac{L}{1-\lambda^{-1} } },
%    \end{equation*}
%    where $L$ is a Lipschitz constant for $f'$.
%\end{rem}

%\begin{rem}
%    When we will use the lemma we always consider tha case of $\sigma = 1$.
%    %without restricting generality.
%\end{rem}




==> exp_lbound.tex <==
We need the following simple lemma from \cite{BEDFORD_HOL}
\begin{lm}   \label{lm:holredef}
    For every \holder function $\omega:I\to \Rb$
    following expression for $h_x(\omega)$ holds
    \begin{gather*}
        h_x(\omega) = \sup \setdef{\gamma}
        { \vmod{\omega(x)-\omega(y)}\leq \vmod{x-y}^\gamma,\ 
        y\in B_\delta(x),\ \delta\geq 0}
    \end{gather*}
\end{lm}

\begin{rem} \label{rem:expexpr}
    It is easy to see that 
    one can replace balls $B_\eps(x)$ 
    in the formula above by any other neighborhoods
    of $x$. In particular the following 
    holds:
    \begin{gather*}
        h_x(\omega) = 
        \sup \setdef
        { \frac{\log\vmod{\omega(x)-\omega(y)}}
        { \log \vmod{x-y} } }
        { y\in B_\delta(x),\ \delta\geq 0}
    %    =
    %    \\
    %    =
    %    \sup \setdef
    %    { \frac{\log\vmod{\omega(x)-\omega(y)}}
    %    { \log \vmod{x-y} } }
    %    { y\in I_{n}(x),\ n\in\Nb}
    %    =
    %    \\
    %    =
    %    \sup \setdef
    %    { \frac{\log\vmod{\omega(x)-\omega(y)}}
    %    { \log \vmod{x-y} } }
    %    { y\in I_{r_i}(x),\ i\in\Nb},
        .
    \end{gather*}
    %where $r_i \to \infty$ as $i\to \infty$.
\end{rem}



It is well known that
 $\mu_\Sigma$ has Gibbs property. 
 I.e. there exists $q>1$ such that
for any $r,m$ and $z\in C_{x_r,\ldots, x_m} $
\begin{equation}
    \label{eq:Gibbs_prop}
    \mu_\Sigma(C_{x_r\ldots x_m} ) 
        \in [q^{-1},q] \exp\enbrace{\sum_{i=0}^{m-r}
         \log a_{x_0}(\sigma^i (z)}
         .
\end{equation}

%\begin{lm}  \label{lm:code_dist}
%    Let $x\in \Sigma$ with
%    $x =  x_1 \ldots x_{m-1} x_{m} \ldots$
%    with $x_{m} \neq n-1$.
%    and $y\in \Sigma$ with
%    $y =  y_1 \ldots y_{m-1} (n-1) \ldots$.
%    Then %$y > x$ and 
%    \begin{equation*}
%        \vmod{\code(y)-\code(x) } \geq \diam  I_{m}(y) .
%    \end{equation*}
%\end{lm}

\begin{lm}  \label{lm:code_dist}
    For $0\leq k,m < r$
    consider $x,x',y\in \Sigma$ such that
    \begin{equation*}
        x =  x_0 \ldots x_{r-k} x_{r-k+1} \ldots x_{r} \ldots x_{r+m-1} x_{r+m} \ldots
    \end{equation*}
    where $x_{r-k} \neq \nbr-1$ and $x_i = \nbr-1$ for $r-k+1\leq i\leq r+m-1$
    and $x_{r+m}\neq \nbr-1$;
    \begin{equation*}
        x' =  x_0 \ldots x_{r-k} x_{r-k+1} \ldots x_{r} \ldots x_{r+m-1} (n-1) \ldots
    \end{equation*}
    and 
    \begin{equation*}
        y =  x_0 \ldots x_{r-k-1} (x_{r-k}+1) 00\ldots 
        .
    \end{equation*}
    Then %$y > x$ and 
    \begin{equation*}
        \dist(x,\code(\cylr_r(x))) = \dist(x, I_r(y) ) \geq \diam  I_{r+m}(x') .
        %\vmod{\code(y)-\code(x) } \geq \diam  I_{r+m}(y) .
    \end{equation*}
\end{lm}

Let $x\in \Sigma$ be such that $x=x_1\ldots x_r\ldots$ and $x_i\neq (\nbr-1)$
for at least one index $0\leq i \leq r$.  
Put $x_r^+ \in \seq{0,\ldots, \nbr-1}^r$ to be
 the next (in lexicographic order) sequence of 
$r$ digits after the sequence formed by first $r$-digits of $x$.
In other words if one views $x_1\ldots x_r$ as a base-$(\nbr-1)$ number,
$x_r^+=x_1\ldots x_r + 0\ldots 0 1$.

Now denote by $\cylr_r(x)$ the next $r$-cylinder to the right of $x$,
i.e. 
\begin{equation*}
    \cylr_r(x) = C_{x_r^+}.
\end{equation*}
One can define $\cyll_r(x)$ analogously.


We will need the following obvious lemma
\begin{lm} \label{lm:exp_from_height}
    Let $x,x',y\in \Sigma$ be like in 
    the Lemma \ref{lm:code_dist}.
    %Let $x\in\Sigma$ and 
    Suppose that  there exist $Z_W,Z_H > 0$
    %such that for a natural number $r$
    %and $y = x_1\ldots x_{r-1} (n-1)\ldots$
    the following inequalities are satisfied:
    \begin{gather*}
        \vmod{E_{r}(x)}_H + \vmod{E_{r}(x_r^+) }_H \leq Z_H, \\
        \vmod{E_{r}(x)}_H + \vmod{E_{r}(x_r^-)}_H \leq Z_H, \\
        \vmod{\diam I_{r+m}(x') } \geq Z_W
    \end{gather*}
    then for any $u_1\in I_r(x)$ and $u_2\in I_r(y)$
    \begin{equation*}
        \frac{\log\vmod{\omega(u_1)-\omega(u_2)}}
        { \log \vmod{u_1-u_2} } 
        %h_x 
        \geq \frac{\log Z_H }{\log Z_W}.
    \end{equation*}
\end{lm}
\begin{proof}
    %Fix $r=r_i$.
    Fix $u_1\in I_r(x)$ and $u_2\in I_r(y)$.
    It is easy to see that 

    [ RLY?? ]

    \begin{gather*}
        \vmod{\alpha(u_1)-\alpha(u_2)} \leq
        \vmod{E_r(x) }_H + \vmod{\cylr_r(x)}_H
        \leq Z_H .
    \end{gather*}
    Lemma \ref{lm:code_dist}
    implies that 
    \begin{equation*}
        \vmod{u_1-u_2} \geq \diam I_{r+m}(x') 
        \geq Z_W .
    \end{equation*}
    Thus 
    %due to Remark \ref{rem:expexpr}.
    \begin{equation*}
        %h_x \geq 
        \frac{\log\vmod{\alpha(u_1)-\alpha(u_2)}}
        { \log \vmod{u_1-u_2} } 
        \geq  \frac{\log Z_H }{\log Z_W} 
        .
    \end{equation*}
    The case of $y\in \cyll_r(x)$ is analogous.
\end{proof}        


\begin{theorem}
    For Lebesgue-almost every $u\in I$
    $h_u(\alpha)\geq \theta$.
\end{theorem}

We will show 
that 
there exist $\eps_0>0$ such that
for Lebesgue-almost every $x$
for every $0<\eps<\eps_0$ 
and every $y\in B_\eps(x)$
the expression
\begin{equation*}
    { \frac{\log\vmod{\omega(x)-\omega(y)}}
    { \log \vmod{x-y} } }
\end{equation*}
is bounded from below by $\theta$.
If we know it then Remark \ref{rem:expexpr}
implies that $h_x(\alpha)\geq \theta$.

Fix a point $x\in I$ with a dense orbit (set of such
$x$ has full measure). 

Fix $\eps>0$ and $y\in B_\eps(x)$, $y\neq x$.
There exists $r\in \Nb$ such that $y$ belongs
either to the right or to the left $r$-cylinder.
Without loss of generality assume 
that $y\in \cylr_{r}(x)$. 
%
%Density of orbit of $x$ implies that
%there exist an infinite number of indices $j$
%such that $x_j = n-1$.
%Fix one such index $j$ such that $j > n_y$.

There are two possibilities:
either $x_r = \nbr -1$ or not.

Suppose first that 
 $x_r = \nbr -1$.
Look at the maximum contiguous block of $(\nbr-1)$'s 
around index $r$.
I.e. consider
 $m = m(x,r) >0 $ -- $1 +$ length of block of $(\nbr-1)$ 
 to the right of $r$'th entry of $x$
 ($1 +$ number of $(\nbr-1)$'s after $x_r$).
and $k = k(x,r)$ -- the same but to the left.

%to estimate exponent of the envelope
%we 
%and estimate $\vmod{\alpha(\code{x})-\alpha(\code{y})}$ 
%from above and together 
%with $\vmod{\code{x}-\code{y}}$ from below.
%
%By Lemma \ref{lm:holredef}
%the following quantity gives 
%a lower bound for the exponent
%\begin{equation*}
%    \frac{\log \vmod{\alpha(\code{x})-\alpha(\code{y})}  }
%    {\log \vmod{\code{x}-\code{y}}}
%\end{equation*}

Put 
\begin{gather*}
    %\xi
     \underline{a} = 
    \min \setdef{a_i(u)}{u\in I,\ 1\leq i <\nbr}, \\
   % \tau = 
    \bar{c} = 
    \max \setdef{ c_i(u) }{ u\in I,\ 0\leq i < \nbr}
\end{gather*}
 and
 $u_i = \code(\sigma^{i}(x))$.

 Put 
 $ I' = I_{r+m} (x_0 \ldots x_{r+m-1} (n-1) \ldots)$.
Lemma \ref{lm:code_dist} %and \ref{lm:width} 
imply that 
\begin{equation*}
    \vmod{\code(x)-\code(y) } \geq 
     \diam I'  
    %\geq a_{x_1} \cdot a_{x_r}
    %\geq M^{-1} \exp (-S_{r+m} f_W(x) ) 
    \geq 
    c_{x_0}(\code(u_0) ) \cdot \ldots 
    \cdot c_{x_{r}}(\code(u_{r}) ) \underline{a}^m
          % just because we contract a unit interval
          % many times
    .
\end{equation*}


%Lemma \ref{lm:height} implies that
%\begin{equation*}
%       \vmod{\alpha(\code{x})-\alpha(\code{y})}
%       \leq \vmod{E_{x_1 \ldots x_r}}_H + \vmod{P_r}_H
%\end{equation*}

Then
\begin{gather*}
    \vmod{E_r(x)}_H + \vmod{\cylr_r(x)}_H 
       \leq N \exp (-S_{r} f_H(x) )  
       + N \exp (-S_{r} f_H(y) )   
       =
       \\
       =
          N
          c_{x_0}(u_0) \cdot \ldots 
          \cdot c_{x_{r-k-1}}(u_{r-k-1}) \cdot
          \\
          \cdot
          \enbrace{ 
              c_{x_{r-k}}(u_{r-k}) \cdot \ldots 
              \cdot c_{x_{r}}(u_{r})
              +
              c_{y_{r-k}}(v_{r-k}) \cdot \ldots 
              \cdot c_{y_{r}}(v_{r})
        }
        \leq 
        \\
       \leq
          N c_{x_0}(u_0) \cdot \ldots 
          \cdot c_{x_{r-k-1}}(u_{r-k-1})  \cdot 2 \bar{c}^k
\end{gather*}
thus if we put
$v_i = \code(\sigma^{i}(y))$
Lemma \ref{lm:exp_from_height} implies that
\begin{gather*}
        \frac{\log\vmod{\omega(x)-\omega(y)}}
        { \log \vmod{x-y} } 
        \geq
  %  \frac{ \log( \vmod{E_{x_1 \ldots x_r}}_H + \vmod{P_r}_H ) }
  %  { \log \diam I_{x_1 \ldots x_{r+m-1} }  }
  %     \geq 
       \frac{ \log ( N c_{x_0}(u_0) \cdot \ldots 
          \cdot c_{x_{r-k-1}}(u_{r-k-1})  \cdot 2 \bar{c}^k ) }
          { 
              \log ( a_{x_0}(u_0) \cdot \ldots 
              \cdot a_{x_{r}}(u_{r}) \underline{a}^m  )
          }
          =
      \\
      =
      \frac{ \sum_{i=0}^{r-k-1}\log (  c_{x_i}(u_i) )  }
          { 
              \sum_{i=0}^{r} \log ( a_{x_i}(u_i) ) 
              + m\log\underline{a}  
          }
          +
       \frac{ \log ( N ) + \log  2 + k\log\bar{c}  }
          { 
        %      \log ( c_{x_1}(u_1) \cdot \ldots 
        %  \cdot c_{x_{r}}(u_{r}) 
              (r+m)\log \underline{a}
          }
\end{gather*}


Now we need to show that the expression 
above convergese to $\theta$ as $r\to \infty$.
Then Remark \ref{rem:expexpr} finishes the proof.

Suppose that we know that 
$m(x,r)/r \to 0$ as $r\to 0$.
%that $k/r \to 0$ and $m/r\to 0$
%as $r\to \infty$ 
Then the second summand tends to $0$ 
and
for the first one we could write
\begin{gather*}
      \frac{ \sum_{i=0}^{r-k-1}\log (  c_{x_i}(u_i) )  }
          { 
              \sum_{i=0}^{r} \log ( a_{x_i}(u_i) ) 
              + m\log\underline{a}  
          }
          =
      \frac{ 
 \frac{1}{r+1} 
 \sum_{i=0}^{r}\log (  c_{x_i}(u_i) )   
        - 
 \frac{1}{r+1} 
        \sum_{i=r-k}^{r}\log (  c_{x_i}(u_i) )  
  }
          {    \frac{1}{r+1} 
              \sum_{i=0}^{r} \log ( a_{x_i}(u_i) ) 
              + \frac{ m}{r+1}\log\underline{a}  
          }
          \geq
          \\
          \geq
      \frac{  \frac{1}{r+1}
        \sum_{i=0}^{r}\log (  c_{x_i}(u_i) )  
        - \frac{k\bar{c}}{r+1}  
      }
          { 
              \frac{1}{r+1}\sum_{i=0}^{r} \log ( a_{x_i}(u_i) ) 
              + \frac{ m}{r+1}\log\underline{a}  
          }
          \to \frac{\int \log c_{u_1}(u) d\mu_\Sigma(u) }
          {\int \log a_{u_1}(u) d\mu_\Sigma(u) }
          = \theta
          .
\end{gather*}

Now we prove that
$m(x,r)/r \to 0$ and $k(x,r)/r\to 0$ as $r\to 0$.
Measure of points with large contiguous blocks 
of a given digit is
small (it follows from the estimate of the measure 
of the cylinder given by the Gibbs property 
\eqref{eq:Gibbs_prop}).
Precisely
\begin{equation*}
    \mu \setdef{x\in\Sigma}
    {\exists r\geq N:\ j_i(x,r)/r \geq \eps}
    \leq \sum_{r=N}^\infty \underline{a}^{r\eps} =
    \underline{a}^{N\eps} \frac{1}{1-\underline{a} }
    \to 0,\ N\to \infty
\end{equation*}
Therefore for $\mu_\Sigma$-almost every $x$  we have that 
$m(x,r)/r \to 0$ as $r\to \infty$.
Consequently for $\Leb$-almost every $y\in I$.


==> explain.tex <==
%\input{explain_old}

This part is to show that a condition on the size of $\lambda$ is unavoidable if
one believes the validity of my estimate 
\eqref{neq:final_lower_bd} (lower bound directly from technical lemmas, we 
do not know if it positive yet).

Let $\eps = 1$.
We need to prove existence of a number $h$ such that 
for every $0\leq j \leq \powk -1 $ the following inequality is satisfied

\begin{gather*}
    0 \geq 
             G_1 h \lambda^{j} 
             +
             \frac{G_2}{ \lambda^{\powk(1-\theta)} } 
             +
        \frac{ G_3 }{ \lambda^{\powk\theta+j}
        h } - G_0,
    \end{gather*}
where
\begin{gather}
    G_0 = \dvcj \\
    G_1=2 \Cdv\\
    G_2 =  \frac{2\maxvprime}{ \lfothk } \\
    G_3 =  \frac{ 2 \maxv }{ \lfthk } 
\end{gather}
and at least for one $j$ the inequality is strict.

    The inequality is equivalent to
    \begin{gather*}
            0 \geq G_1 h^2 \lambda^{j}  \lambda^{\powk(1-\theta)} \lambda^{\powk\theta+j} 
             +
             {G_2} \lambda^{\powk\theta+j} h
             +
        { G_3 } { \lambda^{\powk(1-\theta)} }
        - G_0  \lambda^{\powk(1-\theta)} \lambda^{\powk\theta+j} h =
        \\
        =
             G_1 h^2  \lambda^{j + \powk(1-\theta) + \powk\theta+j} 
             +
             h ( {G_2} \lambda^{\powk\theta+j} 
        - G_0  \lambda^{\powk(1-\theta) + \powk\theta+j} ) +
        { G_3 } { \lambda^{\powk(1-\theta)} }
        =
        \\
        =
            h^2 
            G_1   \lambda^{ \powk+2j} 
             +
             h ( {G_2} \lambda^{\powk\theta+j} 
        - 
        G_0  \lambda^{\powk+j} ) 
        +
        { G_3 } { \lambda^{\powk(1-\theta)} }.
\end{gather*}
It is a quadratic inequality. Denote (for a fixed $j$) the roots
of the corresponding quadratic equation by $h_+,h_-$ and its determinant
by $\mathcal{D}$.

I will show that the roots are real and distinct  (assuming $\powk$ is
large).
Therefore to have inequalities above satisfied for a single $h$ for every $j$
segments bounded by the roots have to intersect.
We shall see that to guarantee it one has to add assumptions like my condition (A).

It is difficult to get nonempty intersection of segments of the most extreme
cases -- when $j=0$ and when $j=\powk-1$.
We shall see that the
interval corresponding to $j=0$ is to the left of the center
of the interval corresponding to $j=\powk-1$, that is
$ h^{(0)}_{+} + h^{(0)}_- >  h^{(\powk-1)}_{+} + h^{(\powk-1)}_- $.

In the end to check that the intersection mentioned above is nonempty.
For this we will look at following inequality
is $h^{(\powk-1)}_+ \geq h^{(0)}_-$. 

First for any $j$ we can write the following
\begin{gather*}
    \frac{h_- + h_+}{2} = \frac{ -{G_2} \lambda^{\powk\theta+j} 
        + 
        G_0  \lambda^{\powk+j} }
        { 2 G_1   \lambda^{ \powk+2j} } ,\\
    \mathcal{D} =  ( {G_2} \lambda^{\powk\theta+j} 
        - 
        G_0  \lambda^{\powk+j} )^2 - 4
            G_1   \lambda^{ \powk+2j} 
        { G_3 } { \lambda^{\powk(1-\theta)} }
        = \\
        =
         {G_2^2} \lambda^{2\powk\theta+2j}  
         -
         2{G_2} G_0 \lambda^{\powk\theta+j}  
          \lambda^{\powk+j}  
        + 
        G_0^2  \lambda^{2\powk+2j}  
        - 
        4 G_1 G_3   \lambda^{ \powk(2-\theta)+2j}  
        = \\
        =
        G_0^2  \lambda^{2\powk+2j}  
        +
         {G_2^2} \lambda^{2\powk\theta+2j}  
         -
         2{G_2} G_0 \lambda^{\powk(1+\theta)+2j}  
        - 
        4 G_1 G_3   \lambda^{ \powk(2-\theta)+2j}  
\end{gather*}


For $j=0$ we have
\begin{gather*}
    \frac{h_- + h_+}{2} = \frac{ -{G_2} \lambda^{\powk\theta} 
        + 
        G_0  \lambda^{\powk} }
        { 2 G_1   \lambda^{ \powk} } = 
        \frac{G_0}{2G_1} - \frac{G_2}{2G_1} \lambda^{-\powk(1-\theta)} 
        ,\\
    \mathcal{D}   
        =
        G_0^2  \lambda^{2\powk}  
        +
         {G_2^2} \lambda^{2\powk\theta}  
         -
         2{G_2} G_0 \lambda^{\powk(1+\theta)}  
        - 
        4 G_1 G_3   \lambda^{ \powk(2-\theta)}   
        ,
        \\
        \sqrt{ \mathcal{D} }
        =
        G_0  \lambda^{\powk}  \sqrt{1 
        +
        \frac{G_2^2}{G_0^2} \lambda^{2\powk\theta-2\powk}  
         -
         2\frac{G_2} {G_0} \lambda^{\powk(1+\theta)-2\powk}  
        - 
        4 \frac{G_1 G_3} {G_0^2}  \lambda^{ \powk(2-\theta)-2\powk}   
    }
    = \\ =
        G_0  \lambda^{\powk}  \enbrace{1 
        +
        \frac{G_2^2}{2G_0^2} \lambda^{2\powk\theta-2\powk}  
         -
         \frac{G_2} {G_0} \lambda^{\powk(1+\theta)-2\powk}  
        - 
        2 \frac{G_1 G_3} {G_0^2}  \lambda^{ \powk(2-\theta)-2\powk}   
    }
    + \mathcal{O}(\lambda^{\powk-2\powk + 2\powk \theta})
%    = \\ =
%      G_0  \lambda^{\powk}   
%        +
%        \frac{G_2^2}{2G_0} \lambda^{2\powk\theta-\powk}  
%         -
%         {G_2}  \lambda^{\powk(1+\theta)-\powk}  
%        - 
%        2 \frac{G_1 G_3} {G_0}  \lambda^{ \powk(2-\theta)-\powk}   
%        + \mathcal{O}
        , 
        \\
        %%%%%%%%%%%%%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%
        \frac{\sqrt{ \mathcal{D} } }{ 2 G_1 \lambda^{\powk} } =
        \frac{G_0}{2G_1}     
        +
        \frac{G_2^2}{4G_0G_1} \lambda^{2\powk\theta-2\powk}  
         -
         \frac{G_2}{2G_1}  \lambda^{\powk(1+\theta)-2\powk}  
        - 
         \frac{ G_3} {G_0}  \lambda^{ \powk(2-\theta)-2\powk}   
         + \\ +
         \mathcal{O} ( %\lambda^{-2\powk(1-\theta)} +
           ( \lambda^{-\powk(1-\theta)} +
            \lambda^{-\powk\theta} )^2 )
\end{gather*}
Here $\mathcal{O}$ denots high order terms in Taylor expansion.

For $j=\powk -1$ we have
\begin{gather*}
    \frac{h_- + h_+}{2} = \frac{ -{G_2} \lambda^{\powk\theta+(\powk-1)} 
        + 
        G_0  \lambda^{\powk+(\powk-1)} }
        { 2 G_1   \lambda^{ \powk+2(\powk-1)} } 
        =
        \frac{ -{G_2} \lambda^{\powk(1+\theta)-1} 
        + 
        G_0  \lambda^{2\powk-1} }
        { 2 G_1   \lambda^{ 3\powk-2} }  
        =  \\ =
        \frac{ G_0   } 
        { 2 G_1    }    \lambda^{2\powk-1 - 3\powk-2}             
        -
        \frac{ {G_2}  } 
        { 2 G_1    }     \lambda^{\powk(1+\theta)-1 -  3\powk-2} 
        =  \\ =
        \frac{ G_0   } 
        { 2 G_1    }    \lambda^{-\powk-3}             
        -
        \frac{ {G_2}  } 
        { 2 G_1    }     \lambda^{\powk(-2+  \theta) - 3} 
        ,\\
    \mathcal{D} 
        =
        G_0^2  \lambda^{2\powk+2(\powk-1)}  
        +
         {G_2^2} \lambda^{2\powk\theta+2(\powk-1)}  
         -
         2{G_2} G_0 \lambda^{\powk(1+\theta)+2(\powk-1)}  
        - 
        4 G_1 G_3   \lambda^{ \powk(2-\theta)+2(\powk-1)}  
        =\\=
        G_0^2  \lambda^{4\powk-2}  
        +
         {G_2^2} \lambda^{\powk(2+2\theta)-2}  
         -
         2{G_2} G_0 \lambda^{\powk(3+\theta)-2}  
        - 
        4 G_1 G_3   \lambda^{ \powk(4-\theta)-2}  
        , \\
        \sqrt{ \mathcal{D} } = 
        G_0  \lambda^{2\powk-1} \sqrt{ 1
        +
        \frac{G_2^2}{G_0^2} \lambda^{\powk(2+2\theta)-2 - 4\powk+2}  
         -
         2\frac{G_2}{G_0} \lambda^{\powk(3+\theta)-2- 4\powk+2}  
        - 
        4 \frac{G_1 G_3}{G_0^2}   \lambda^{ \powk(4-\theta)-2- 4\powk+2}  
    } 
    = \\ =
        G_0  \lambda^{2\powk-1} \sqrt{ 1
        +
        \frac{G_2^2}{G_0^2} \lambda^{\powk(-2+2\theta)}  
         -
         2\frac{G_2}{G_0} \lambda^{\powk(-1+\theta)}  
        - 
        4 \frac{G_1 G_3}{G_0^2}   \lambda^{ \powk(-\theta)}  
    } 
    = \\ =
        G_0  \lambda^{2\powk-1} \enbrace{ 1
        +
        \frac{G_2^2}{2G_0^2} \lambda^{\powk(-2+2\theta)}  
         -
         \frac{G_2}{G_0} \lambda^{\powk(-1+\theta)}  
        - 
        2 \frac{G_1 G_3}{G_0^2}   \lambda^{ \powk(-\theta)}  
    } 
    + \\ +
     \mathcal{O} 
     \enbrace{ \lambda^{2\powk-1}
     (
         \lambda^{-2\powk(1-\theta)}  
         +
          \lambda^{-\powk(1-\theta)}  
        + 
           \lambda^{ -\powk\theta}  )^2
    }
    , \\
        %%%%%%%%%%%%%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%
        \frac{\sqrt{ \mathcal{D} } }{ 2 G_1 \lambda^{3\powk-2} } =
        \frac{G_0}{2G_1}  \lambda^{-\powk+1} \enbrace{ 1
        +
        \frac{G_2^2}{2G_0^2} \lambda^{\powk(-2+2\theta)}  
         -
         \frac{G_2}{G_0} \lambda^{\powk(-1+\theta)}  
        - 
        2 \frac{G_1 G_3}{G_0^2}   \lambda^{ \powk(-\theta)}  
         + \mathcal{O}
    } 
    = \\ =
        \frac{G_0}{2G_1}  \lambda^{-\powk+1} 
        +
        \frac{G_2^2}{4G_0 G_1} \lambda^{\powk(-2+2\theta)-\powk+1}  
         -
         \frac{G_2}{2G_1} \lambda^{\powk(-1+\theta)-\powk+1}  
        - 
         \frac{ G_3}{G_0}   \lambda^{ \powk(-\theta)-\powk+1}  
         + \mathcal{O}
    = \\ =
        \frac{G_0}{2G_1}  \lambda^{-\powk+1} 
        +
        \frac{G_2^2}{4G_0 G_1} \lambda^{\powk(-3+2\theta)+1}  
         -
         \frac{G_2}{2G_1} \lambda^{\powk(-2+\theta)+1}  
        - 
         \frac{ G_3}{G_0}   \lambda^{ \powk(-1-\theta)+1}  
         +\\+
         \mathcal{O} \enbrace{ (
             \lambda^{-\powk(3-2\theta)}  
             +
              \lambda^{-\powk(2-\theta)}  
            + 
              \lambda^{ -\powk(1+\theta)} )^2  
         }
\end{gather*}

We see that $h_-^{(0)} + h_+^{(0)} > h_-^{(\powk-1)} + h_+^{(\powk-1)} $.

After all we need
\begin{gather*}
    0 < h_+^{(\powk-1)} - h_-^{(0)} 
    =
        \frac{ G_0   } 
        { 2 G_1    }    \lambda^{-\powk-3}             
        -
        \frac{ {G_2}  } 
        { 2 G_1    }     \lambda^{\powk(-2+  \theta) - 3} 
    +   \\ +
        \frac{G_0}{2G_1}  \lambda^{-\powk+1} 
        +
        \frac{G_2^2}{4G_0 G_1} \lambda^{-\powk(3-2\theta)+1}  
         -
         \frac{G_2}{2G_1} \lambda^{-\powk(2-\theta)+1}  
        - 
         \frac{ G_3}{G_0}   \lambda^{ -\powk(1+\theta)+1}  
         + \mathcal{O}_1
         %%%%%%%%%%%%%%%%%%
        - \\ -
        \enbrace{ \frac{G_0}{2G_1} - \frac{G_2}{2G_1} \lambda^{-\powk(1-\theta)} 
      -
        \frac{G_0}{2G_1}     
        -
        \frac{G_2^2}{4G_0G_1} \lambda^{-\powk(2-2\theta)}  
         +
         \frac{G_2}{2G_1}  \lambda^{-\powk(1-\theta)}  
        + 
         \frac{ G_3} {G_0}  \lambda^{ -\powk\theta}   
        + \mathcal{O}_2
    }
    =  \\ =
        \frac{ G_0   } { 2 G_1    }    \lambda^{-\powk-3}             
        +
        \frac{G_0}{2G_1}  \lambda^{-\powk+1} 
     %   +
     %   \frac{G_2^2}{4G_0 G_1} \lambda^{-\powk(3-2\theta)+1}  
     %   + 
     %      \frac{G_2}{2G_1} \lambda^{-\powk(1-\theta)} 
        +
        \frac{G_2^2}{4G_0G_1} \lambda^{-2\powk(1-\theta)}  
        - \\ 
       % -
      %  \frac{ {G_2}  } { 2 G_1    }     \lambda^{\powk(-2+  \theta) - 3} 
         -
         \frac{G_2}{2G_1} \lambda^{-\powk(2-\theta)+1}  
        - 
         \frac{ G_3}{G_0}   \lambda^{ -\powk(1+\theta)+1}  
         %%%%%%%%%%%%%%%%%%
       %  -
       %  \frac{G_2}{2G_1}  \lambda^{-\powk(1-\theta)}  
        - 
         \frac{ G_3} {G_0}  \lambda^{ -\powk\theta}   
        + \mathcal{O}_2
         + \mathcal{O}_1
         = \\ = 
         \lambda^{-\powk} 
         \enbrace{
        \frac{ G_0   } { 2 G_1    }    \lambda^{-3}             
        +
        \frac{G_0}{2G_1}  \lambda 
     %   +
     %   \frac{G_2^2}{4G_0 G_1} \lambda^{-\powk(3-2\theta)+1}  
     %   + 
     %      \frac{G_2}{2G_1} \lambda^{\powk\theta} 
        +
        \frac{G_2^2}{4G_0G_1} \lambda^{-\powk(1-2\theta)}  
    }
        - \\ -
         \lambda^{-\powk} 
         \enbrace{
        %\frac{ {G_2}  } { 2 G_1    }     \lambda^{\powk(-2+  \theta) - 3} 
        % +
         \frac{G_2}{2G_1} \lambda^{-\powk(1-\theta)+1}  
        + 
         \frac{ G_3}{G_0}   \lambda^{ -\powk\theta+1}  
         %%%%%%%%%%%%%%%%%%
     %    +
     %    \frac{G_2}{2G_1}  \lambda^{\powk\theta}  
        + 
         \frac{ G_3} {G_0}  \lambda^{ \powk(1-\theta) }   
     }
        + \mathcal{O}_2
         + \mathcal{O}_1
\end{gather*}

Due to the presence of the last summand 
$ \frac{ G_3} {G_0}  \lambda^{ \powk(1-\theta) }   $
with positive $\powk$-multiple power of $\lambda$
one has to impose an additional condition to get positivity of this expression.

The condition is essentialy that
\begin{gather*}
    \frac{G_0}{2G_1} \lambda^{-3} + \frac{G_0}{2G_1}\lambda \geq 
    \frac{G_3}{G_0} \lambda^{\powk(1-\theta) }
\end{gather*}
i.e.
\begin{gather*}
     \lambda^{\powk(1-\theta) }
    \leq
 \frac{G^2_0}{2G_3 G_1} \enbrace{ 
     \frac{1}{\lambda^{3}} + \lambda   }
\end{gather*}

This condition
prevents $k_0$ to be too big. 
Probably it is possible to write it accurately 
talking care about 
$\mathcal{O}$ terms as well (because formally although
there is nothing in these terms that would allow to kill 
$\lambda^{\powk (1- \theta)}$ summand, 
there are something that would enter the condition)
and rephrase the condition (A). 
However quanitatively it would still be
the same, requiring nontrivial relation between sizes of $\powk,\lambda$
and $v$-related contstants.

Then under (an accurate version of) this condition 
it would be possible to prove a lower bound in the theorem without
assuming that some terms are less than a third of another.
However I do not think somebody might need the best possible
exact expression for this lower bound.
%which would make output even more ugly.

To be completely precise one has to take into account that $G_0$ depends on $j$
but it does not change the overall picture.

\newpage


==> explain_old.tex <==
Let $\eps = 1$.
We need the existence of $h$ such that 
for every $0\leq j \leq \powk -1 $ the following inequality to be satisfied
\begin{equation*}
        G_0
            -
             G_1 h \lambda^{j}
        -
             \frac{G_2}{ \lambda^{\powk(1-\theta)} } 
             -
        \frac{ G_3 }{ \lambda^{\powk\theta+j}
        h }
        > 0,
\end{equation*}
where
\begin{gather}
    G_0 = \dvcj \\
    G_1=2 \Cdv\\
    G_2 =  \frac{2\maxvprime}{ \lfothk } \\
    G_3 =  \frac{ 2 \maxv }{ \lfthk } 
\end{gather}
Assume that $\powk$ is very big and try to solve inequality
\begin{equation*}
        G_0 - G_1 h \lambda^{j}
             - \frac{ G_3 }{ \lambda^{\powk\theta+j}
        h }
        > 0.
\end{equation*}
It is equivalent to 
\begin{equation*}
        h^2 G_1 \lambda^{2j + \powk\theta }
             - h G_0  \lambda^{\powk\theta+j}
             +  G_3 
        < 0.
\end{equation*}
It is a quadratic inequality
with roots of the corresponding equation
\begin{gather*}
    \mathcal{D}_j = 
    G_0^2 \lambda^{2\powk \theta + 2j} - 
    4 G_1 G_3 \lambda^{\powk \theta + 2j}
    \\
    h^{(j)}_{\pm} = \frac{ G_0 \lambda^{\powk \theta+j} \pm 
    \sqrt{ \mathcal{D}_j } }{2G_1\lambda^{\powk\theta+2j}}
\end{gather*}
As we supposed that $\powk$ is big, $\mathcal{D}$ is positive.

Now we have
\begin{gather*}
    h^{(0)}_{+} + h^{(0)}_- = \frac{ G_0   } {2G_1} 
    \\
    h^{(\powk-1)}_{+} + h^{(\powk-1)}_- = 
    \frac{ G_0   } {2G_1\lambda^{\powk-1} }   \\
    %
    %
    \frac {\sqrt{ \mathcal{D}_0 } }{2G_1\lambda^{\powk\theta}} 
    = \frac{ \sqrt{ G_0^2 \lambda^{2\powk \theta } - 
    4 G_1 G_3 \lambda^{\powk \theta } } }{2G_1\lambda^{\powk\theta}} 
    = \frac{ \sqrt{ G_0^2  - 
    4 G_1 G_3 \lambda^{-\powk \theta } } }{2G_1} 
    \\
    \frac {\sqrt{ \mathcal{D}_{\powk-1} } }{2G_1\lambda^{2(\powk-1)+\powk\theta}} 
    =
    \frac{
    \sqrt{ G_0^2 \lambda^{2\powk \theta + 2(\powk-1)} - 
    4 G_1 G_3 \lambda^{\powk \theta + 2(\powk-1)} } 
        }{2G_1\lambda^{\powk\theta+2(\powk-1)}}
        =
    \frac{
    \sqrt{ G_0^2 \lambda^{- 2(\powk-1)} - 
    4 G_1 G_3 \lambda^{-\powk \theta - 2(\powk-1)} } 
        }{2G_1}
\end{gather*}



As $ h^{(0)}_{+} + h^{(0)}_- >  h^{(\powk-1)}_{+} + h^{(\powk-1)}_- $ 
and we need all the intervals of negativity to intersect, 
we have to check that
is $h^{(\powk-1)}_+ > h^{(0)}_-$ i.e.
\begin{gather*}
    \frac{ G_0   } {2G_1\lambda^{\powk-1} }   
    + \frac{
    \sqrt{ G_0^2 \lambda^{- 2(\powk-1)} - 
    4 G_1 G_3 \lambda^{-\powk \theta - 2(\powk-1)} } 
        }{2G_1}
    - \frac{ G_0   } {2G_1}  +
     \frac{ \sqrt{ G_0^2  - 
    4 G_1 G_3 \lambda^{-\powk \theta } } }{2G_1}  > 0
\end{gather*}
Unfortunately here we have a problem. If we just make $\powk$ very large,
firt and second summands dissapears and the fourth one is not large enough to
compensate the negativity of the third summand.

One can than do a Taylor expansion for the third summand and that expect that
the first summand would help. It does but only if one assumes certain relation between
$G_0,G_1, G_3$. This relation is very similar to the the one I have in my condition (A).


==> hcond.tex <==
  %  Let $N_h$ be a natural number,  $h_0>0$
  %  and $h>0$ be such that
    \begin{gather*} % \label{eq:Ndef_nlin_lm}
        \frac{  h_0}{ 2\Cbdistort \dfxx{N_h+1}{x} } \leq h \leq
        \frac{  h_0 }{ 2\Cbdistort \dfxx{N_h}{x} }   
        .
    \end{gather*}


==> hcond_lin.tex <==

    %Under the conditions of the Theorem
    Let $N_h$ be a natural number,  $h_0>0$
    and $h>0$ be such that
    \begin{gather*}  %\label{eq:Ndef_lin_lm}
       %\frac{1}{ \dfxth{N} }  
        \frac{ h_0}{ 2\lambda^{N_h} } \leq h \leq
        \frac{ h_0 }{ \lambda^{N_h} }  
        .
    \end{gather*}


==> lbd_separate_prop.tex <==
\begin{prop}  
   % if $(f,v)$ satisfy condition (A) at point $c$
    Let $\powk>0$ be a natural number and $0 \leq j \leq \powk -1 $
    If $c$ is a $\powk$-periodic point of $f$
    such that $\dvcj > 0$
        then
        for every $\hat{h}>0$,
        every $\delta_1<\delta_2$,
        every natural $N > \powk$
        such that $\lambda^{-(\powk N + \powk-1)} \delta_2 < \hat{h}$,
        every $N$-th preimage $x$ of $c$
        and
        every $h$ such that
        \begin{equation*}
        \frac{ \delta_1 }{ \lambda^{\powk N}  } \leq h \leq
        \frac{ \delta_2 }{ \lambda^{\powk N}  }    
        \end{equation*}
        the following lower bound holds: 
        \begin{gather*}
            \vmod{\alpha(x)-\alpha(x+h)}
            h^{-\theta}
            \geq 
            \sum_{j=0}^{\powk}
            ({\delta^{(j)}_1)^{1-\theta}}
            {\lambda^{j(1-\theta)-\theta}  } 
            \enbrace{
            \dvcj
            -
            2\Cdvj (\delta^{(j)}_2)^\eps \lambda^{j\eps}
            -
            \frac{4\maxvprime}{\lambda^{\powk(1-\theta)} } 
            -
            \frac{ 8 \maxv }{ \lambda^{\powk\theta+j}
        \delta^{(j)}_1 }
    }
    \end{gather*}
        where $\Cdvj$ is a local $\eps$-\holder constant at $f^j(c)$
\end{prop}



==> lower_bound_lin_small_lbd.tex <==
\begin{lm} \label{lm:lin_lower_bd_smalllbd}
    Let $N$ be a natural number, $0\leq j\leq \powk-1$,
    $0<\delta_1,\delta_2\leq 1$, $\delta>0$ 
    and $h>0$ be such that
    \begin{gather*}  %\label{eq:Ndef_lin_lm}
        \frac{ \delta_1}{ \lambda^{\powk N} } \leq h
        \leq
        \frac{ \delta_2 }{ \lambda^{\powk N} }  
        .
    \end{gather*}
    If $x,c\in\mfd$ are 
    such that
    $ \dist(f^{j + \powk N}(x), f^j(c) ) \leq \delta$,
    and
    $ v'(f^{j}(c)) > 0$
    then
    \begin{gather*}
        h^{-\theta}
        \frac{\lambda^{\theta} }{ \delta_1^{1-\theta} \lambda^{j(1-\theta)}  } 
        \vmod{ S^{(j)}_{0,N}(x,h) }
        \geq
        {v'(f^{j}(c))} 
            -
 \Cdvtmp \delta_2^\eps \lambda^{j\eps} 
                    -
                    \Cdvtmp \delta^\eps 
        -
             \frac{2\maxvprime}{(\lfothk)\lambda^{\powk(1-\theta)} } 
    \end{gather*}
    where $\Cdvtmp$ is a local $\eps$-\holder constant for $v'$ at $f^{j+N\powk}(x)$.
\end{lm}

%\textbf{
%    [
%        The reason because we have additional  $\lambda^{j(1-\theta)}$ appearing
%is that 
%in the linear case we can write
%\begin{gather*}
%    \lambda^{-\theta} S_{0,N}^{(j)}(x,h) =
%    \lambda^{-j\theta-\theta} S_{0,N}^{f=f^\powk}(f^j(x),\lambda^j h)
%\end{gather*}
%I could write a proof of this lemma out of it, but 
%I would like to keep it as it is to be able to repeat in the nonlinear case
%(because the last formula does not work there)
%\\
%Also this formula (the fact that it has $\lambda^j h$ instead of $h$ on the right
%side) show that my naive initial idea that
%a kind of ergodic theorem (that was replaced by your idea to look
%only at periodic points)
%would help to rule everything out without imposing additional restrictions
%on properties of $f$ and $v$, was wrong.
%] }

\begin{proof}[Proof of the lemma] 

        Note that
        using the upper bound on $h$
        we obtain for certain $\xi\in (x,\xi_N) \subset (x,x+h)$
    \begin{gather*}
        \vmod{ v'(f^{j+ \powk N}(\xi_N)) - 
        v'(f^{j+\powk N}(x)) }
        \leq  
        \Cdvtmp \vmod{ f^{j+ \powk N}(\xi_N) - f^{ j +\powk N}(x) }^\eps
        =
        \\
        =
        \Cdvtmp \vmod{ \dfxx{j + \powk N}{\xi} (\xi_N - x)}^\eps 
        =
        \Cdvtmp (\lambda^{j+\powk N} h)^\eps \leq \Cdvtmp \lambda^{j\eps} \delta_2^\eps
    \end{gather*}

    Using the lower bound for $h$, estimate \eqref{eq:vDiff}
    and the condition on $x$
    we can write the following estimates:
    \begin{gather*}
        h^{-\theta}
        \frac{\lambda^{\theta} }{ \delta_1^{1-\theta}} 
        \vmod{ S_{0,N}^{(j)}(x,h) }
        =
        h^{1-\theta} 
        \frac{\lambda^{\theta} }{ \delta_1^{1-\theta}} 
        \vmod{
             \frac{1}{\lambda^\theta} \sum_{i=0}^n 
        v'( f^{j + \powk i }(\xi_i) )   \lambda^{ (j+\powk i)(1-\theta)} 
             } \geq 
            %%%%%%%%%%%%% 2%%%%%%%%%%%%%%%%%%%%%%%%
        \\
        \geq
            \vmod{
                \sum_{i=0}^{N} v'(f^{j+\powk i}(\xi_i))
            \frac{  1 }
            {  \lambda^{(-j +(N- i)\powk)(1-\theta)}  } }    
            \geq 
            \\
        \geq
        { \vmod{ v'(f^{j+\powk N}(\xi_N)) } } \lambda^{j(1-\theta)}
                -
                    \sum_{i=0}^{N-1} 
            \frac{  \vmod{ v'(f^{j+\powk i}(\xi_i)) }  }
            {  \lambda^{(-j + (N-i) \powk)(1-\theta)}  }     
            \geq 
            \\
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \geq  
        \vmod{v'(f^{j+\powk N}(x))} \lambda^{j(1-\theta)} -
        \Cdvtmp \delta_2^\eps \lambda^{j(1-\theta+\eps )}
        -
             \frac{2\maxvprime}{(\lfothk)\lambda^{(\powk-j)(1-\theta)}
          } 
          .
    \end{gather*}

\end{proof}



==> prep_nonhol.tex <==

    Fix a point $x$ such that
    trajectory of every point $f^i(x),\ i=0\dots \powk-1$ 
    is dense under the action fo $f^{\powk}$.

    The set of such points $x$ has full Lebesgue measure 
    because of ergodicity of $f$
    with respect to an invariant measure $\mu$ having  
    positive density $\frac{d\mu}{d\Leb}$
   % (in fact denseness of the orbit of almost every point 
   % is enough).

    We will show that 
    %there exists $C_0>0$ such that
    for every $\hat{h}>0$
    %for Lebesgue-almost every point $x\in \mfd$
    there exists
    $0<h<\hat{h}$ %(by choosing $N$ large enough)
    so that 
    \begin{equation*}
         \frac{ \vmod{\alpha(x+h) - \alpha(x) } }{ h^{\theta} } 
        \geq C_0/2.
        %\tobeless ,
    \end{equation*}                                    
%    where $\tobeless$ is a constant (to be defined later) depending only
%    on $f$ and $\theta$.

    Fix $\hat{h}>0$.

    Take $0<\delta$ such that
    \begin{equation*}
        \Cdv\delta^\eps < \maxvprime \xi /10.
    \end{equation*}

    Choose positive integer $N = N(x)$ be such that
    \begin{gather}
        \dist(\lambda^{N+1}  , c ) < \delta , 
        \label{eq:Nofdeltadef} \\
        \lambda^{-N} < \hat{h}.  \nonumber
    \end{gather}


    We also choose $h > 0$ such that 
    \begin{gather}  \label{eq:Ndef}
        \frac{ 1}{ \lambda^{N+1}  } \leq h \leq
        \frac{ 1 }{ \lambda^{N}  }    
        .
    \end{gather}



==> prooflin_small_lbd.tex <==
\subsection{Proof of the lower bound in the linear case, general $\powk$}

For a natural $\powk \geq 1$
    for every 
    $x$ from $S^1$ and $h>0$
 we can rewrite the formula \eqref{eq:cohomSolFormula} as
\begin{gather*}
    \alpha(x) = - \sum_{j=0}^{\powk-1}
    \sum_{i=0}^{\infty} \frac{v(f^{\powk i+j}(x)) }{ \dfxth{\powk i+j+1} }
    .
\end{gather*}

Therefore
\begin{gather*}
    \alpha(x) - \alpha(x+h) =
    \sum_{j=0}^{\powk-1}  B_j(x,h) 
\end{gather*}
where
\begin{gather*}
    %\label{eq:alphapart}
    B_j(x,h) =  %h^{-\theta}\enbrace{
        {
        \sum_{i=0}^{\infty} \frac{v(f^{\powk i+j}(x)) }{ \dfxthx{\powk i+j+1}{x} } 
    -
    \sum_{i=0}^{\infty} \frac{v(f^{\powk i+j}(x+h)) }{ \dfxthx{\powk i+j+1}{x+h}} 
}
=
\\
        %%%%%%
        = \sum_{i=0}^{\infty}
        \frac{1}{\lambda^{\theta (j+\powk i+1)} }
        \enbrace{v(f^{j+\powk i}(x+h)) -v(f^{j+\powk i}(x))}   .
    %\label{eq:alphadif_lin_smalllbd} 
    \end{gather*}


    For $n\in \Zplus$ and $m \in \Zplusinf$ such that $n\leq m$
    we introduce the following notation:
    \begin{equation*}
        S^{(j)}_{n,m}(x,h) = 
 \sum_{i=n}^{m} \frac{1}{\lambda^{(j + \powk  i+1)	\theta} }
 \enbrace{v(f^{j+\powk i }(x+h)) -v(f^{j+\powk i}(x))}     .
    \end{equation*}

    Note that for every $0\leq j \leq \powk-1$ for every natural number $n$ there
    exist $\xi_i\in (x,x+h)$ for $0\leq i\leq n$
    such that
    \begin{gather*}
        S_{0,n}^{(j)}(x,h) = \frac{h}{\lambda^{\theta}} \sum_{i=0}^n 
        v'( f^{j + \powk i}(\xi_i) )   \lambda^{(j+\powk i)(1-\theta)}
    \end{gather*}


    \subsubsection{Technical lemmas}
    \input{tail_estim_lin_small_lbd}
    \input{lower_bound_lin_small_lbd}

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%    \subsection{Lower bound}
    
    Assume that condition (A) is satisfied for 
    a point $c$ and $\powk\geq 1$.
    Suppose without restricting generality that $v'(c)>0$ (this
    implies that $\dvcj > 0$ for every $0\leq j\leq \powk-1$ by condition (A) ).


    Fix $\hat{h}$.
    We first give expressions for $\delta_1,\delta_2$
    that depend only on $f,v$ and $\powk$
    and later
    select $x$, $N$ and $h = h(N,\delta_1,\delta_2) < \hat{h}$
    such that $ \vmod{\alpha(x) - \alpha(x+h) } / h^\theta$ 
    has a positive lower bound.

    For every
    $0<\delta^{(j)}_1,\delta^{(j)}_2 \leq 1$
    for every $x$ for which  
    there exists a natural number $N>\powk$ such that
    \begin{equation*}
        \vmod{f^{\powk N}(x) - c} < 
        \delta^{(j)}_2 \lambda^{-\powk+1}
        ,
    \end{equation*}
    lemmas \ref{lm:lin_supp_bounds_smalllbd} and
    \ref{lm:lin_lower_bd_smalllbd} for $\delta=\delta_2 \lambda^j$ imply that
        for every
        $h = h(N)$ such that 
    \begin{gather*} % \label{eq:Ndef}
        \frac{ \delta^{(j)}_1 }{ \lambda^{\powk N}  } \leq h \leq
        \frac{ \delta^{(j)}_2 }{ \lambda^{\powk N}  }    
    \end{gather*}
    the following bound holds for every $0\leq j\leq \powk-1$:
        \begin{gather}
            B_j(x,h) 
             { (\delta^{(j)}_1)^{\theta-1}}
            {\lambda^{-j(1-\theta)+\theta}  } 
         h^{-\theta}
        \geq      \nonumber
        \\
        \geq
        \dvcj
            -
            2 \Cdv (\delta^{(j)}_2)^\eps \lambda^{j\eps}
        -
             \frac{2\maxvprime}{ (\lfothk)\lambda^{\powk(1-\theta)} } 
             -
        \frac{ 2 \maxv }{ (\lfthk)\lambda^{\powk\theta+j}
        \delta^{(j)}_1 }
        .
        \label{neq:final_lower_bd}
        \end{gather}
        %where $\Cdvj$ is a local $\eps$-\holder constant for $v'$ at $f^j(c)$
        Note that the right-hand side of 
        this expression does not depend on $x,N$ and $h$.

        
        It is possible to choose $\delta^{(j)}_1,\delta^{(j)}_2>0$ in such a way
    that the expression above is greater than zero.
    %
    To guarantee that the second and the third summands in the right-hand
    side of \eqref{neq:final_lower_bd} are both less than
    $\dvcj/3$ it is enough to put 
    \begin{gather*}
        \delta^{(j)}_1 \leq D^{(j)}_1 =
            \frac{6 \maxv}{(\lfthk)\dvcj   \lambda^{\powk\theta + j}}, \\
        \delta^{(j)}_2 \geq D^{(j)}_2 =
            \enbrace{ \frac{\dvcj}{6\Cdv}}^{1/{\eps}}
        \frac{1}{\lambda^{j } }
    \end{gather*}

    To be able to select $\delta_1$ and $\delta_2$ in such a way
    so that
    they satisfy the bounds above
    %give positive expression
    for every $j$
    but do not depend on $j$,
    we use inequality \eqref{neq:A_bd1} from condition (A).
    It implies that 
    \begin{equation*}
        \frac{6\maxv}{ (\lfthk) \mindvcj \lambda^{\powk \theta} }
        =  \max_j D^{(j)}_1 \leq
        \min_j D^{(j)}_2
        =
        \enbrace{ \frac{\mindvcj  }{6\Cdv} }^{1/\eps} 
        \frac{1}{\lambda^{\powk-1}}
        ,
    \end{equation*}
    where
    \begin{gather*}
        \mindvcj = \min_{0 \leq j \leq \powk-1} {v'(f^j(c))}
        .
    \end{gather*}


    Put $\delta_1 = \max_j D_1$ and $\delta_2 = \min_j D_2$.
    Inequality \eqref{neq:A_bd3} from condition (A) 
    implies that $\delta_2 \leq 1$.

    Now fix a point $x$ such that there exists
    a natural $N$ such that
    \begin{gather*}
        \vmod{f^{\powk N}(x) - c} < 
        \delta_2 \maxdf^{-\powk+1}, \nonumber \\
        \delta_2 \lambda^{-\powk N} < \hat{h}
        .
    \end{gather*}
    One can take $x$ to be a point from
    the $\powk N$'th-preimage of $B_{\delta_2}(c)$ for sufficiently large $N$ or
    any point with a
    dense trajectory (the set of which has full Lebesgue measure).
    In the latter case $x$ does not depend on $\hat{h}$.

    Now inequality \eqref{neq:A_bd2} from condition (A)
    and the definition of $\delta_1,\delta_2$
    allow us to select a (single) $h < \hat{h}$ such that 
    expression \eqref{neq:final_lower_bd} is larger than
    $\dvcj / 12$ for every $j$.

    Finally
    \begin{equation*}
        \frac{ \vmod{ \alpha(x) - \alpha(x+h) } } { h^\theta}
        \geq C_0 > 0
    \end{equation*}
    for 
    \begin{gather*}
        C_0  =
        \delta_1^{1-\theta} 
        \frac{1}{12}\sum_{j=0}^{\powk -1 } \dvcj \lambda^{-j(1-\theta) + \theta}
        =
        \\
        =
        \enbrace{ \frac{6\maxv}{ (\lfthk)
            \mindvcj \lambda^{\powk \theta} } }^{1-\theta}
        \frac{1}{12}\sum_{j=0}^{\powk -1 } \dvcj \lambda^{-j(1-\theta) + \theta}
        .
    \end{gather*}
    In particular, $C_0$ does not depend on $h$.


==> tail_estim_lin_small_lbd.tex <==
\begin{lm}                         \label{lm:lin_supp_bounds_smalllbd}
    Let $N$ be a natural number, $0\leq j\leq \powk-1$, 
    $0<\delta_1<1$
    and $h>0$ be such that
    \begin{gather*}  %\label{eq:Ndef_lin_lm}
        \frac{ \delta_1}{ \lambda^{\powk N} } \leq h 
        .
    \end{gather*}

    Then 
    for every $x\in\mfd$ the following estimate holds:
\begin{gather*}
    \vmod{S_{N+1,\infty}^{(j)}(x,h) }
  \leq
  \frac{ 2 \maxv }{ (\lfthk) \lambda^{(j+1+\powk)\theta} \delta_1^{\theta} }
        h^\theta  
  \end{gather*}

\end{lm}
\begin{proof}[Proof of the lemma]
    We may easily estimate the tail
    of ${S_{0,\infty}}$ using the lower bound on $h$:
    \begin{gather*}
        \vmod{S_{N+1,\infty}^{(j)}(x,h) }  \leq
        2\maxv \frac{1}{\lambda^{(j+(N+1) \powk +1 )\theta}}
        \sum_{i=0}^{\infty}  \lambda^{-i \powk\theta} 
        \leq
        \\
        \leq
        \frac{2\maxv}{(1 - \lambda^{-\powk\theta}) \lambda^{(j+(N+1) \powk +1) \theta} }
        \leq 
        \frac{2 \maxv}{\lfthk}
        \lambda^{-(j+1+\powk)\theta} \delta_1^{-\theta} h^\theta .
    \end{gather*}


\end{proof}



==> uniquesol_no_r.tex <==

    To prove that it is the only bounded solution, suppose there is another 
    bounded solution $\beta$.
    We do the proof for $\prexp = 1$ but in general case the changes are minimal.
    For $K = \max(\sup \vmod{\alpha}, \sup \vmod{\beta})$
    take $N\in\Nb$ so that 
    \begin{equation*}
        \frac{K}{\dfxth{N}} < \vmod{\beta(x) - \alpha(x) } / 3 .
    \end{equation*}

    Note that for $\alpha$
    we can write a finite analog of solution forumla \eqref{eq:cohomSolFormula}:
    \begin{gather*}
        \alpha(x) = \frac{-v(x) }{ \dfxthxp{x} }  +
        \frac{\alpha(f(x)) }{ \dfxthxp{x}}
        =      \nonumber
        \\
        =\frac{-v(x) }{ \dfxthxp{x} }  
        + \frac{1 }{ \dfxthxp{x} } 
        \enbrace{\frac{-v(f(x)) }{ \dfxthxp{f(x)} }  +
        \frac{\alpha(f^2(x)) }{ \dfxthxp{f(x)} } } = 
        \nonumber
        \\
        =\frac{-v(x) }{ \dfxthxp{x}  }  -  
        \frac{v(f(x)) }{ \dfxth{2}  }  +
        \frac{\alpha(f^2(x)) }{\dfxth{2}}  = \ldots =  
        \nonumber
        \\
        =-\sum_{i=0}^{N-1} \frac{v(f^i(x)) }{ \dfxth{i+1} } +
        \frac{\alpha(f^N(x)) }{ \dfxth{N} }.
     %   \label{eq:finite_alpha_rep}
    \end{gather*}

    Analogously 
    \begin{gather*}
%        \alpha(x) = -\sum_{i=0}^{N-1} \frac{v(f^i(x)) }{ \dfxth{i+1} } +
%        \frac{\alpha(f^N(x)) }{ \dfxth{N} }; \\
%%
        \beta(x) = -\sum_{i=0}^{N-1} \frac{v(f^i(x)) }{ \dfxth{i+1} } +
        \frac{\beta(f^N(x)) }{ \dfxth{N} }.
    \end{gather*}
    Then 
    \begin{equation*}
        \frac{3K}{ \dfxth{N}} < \vmod{\alpha(x) - \beta(x) }= 
        \vmod{ \frac{  \alpha(f^N(x)) - \beta(f^N(x)) }
        { \dfxth{N} } } \leq \frac{2K}{  \dfxth{N} },
    \end{equation*}
    which is  a contradiction.
    %because $\vmod{\alpha(x) - \beta(x)} \leq 2K / \dfxth{N}$.


==> upper_bound.tex <==
\begin{lm}     \label{lm:nlin_upper_bd} 
    \input{hcond}
    Then
    for $N \leq N_h$
    \begin{gather*}
        h^{-\theta} \vmod{ \hat{S}_{N} } 
        \leq
                    \frac{4\maxvprime
                        }
                     { \lambda^{(N_h-N)(1-\theta)+\theta } }
        \enbrace{\frac{h_0}{2\Cbdistort}}^{1-\theta}
    \end{gather*}
\end{lm}

\begin{proof}
    Using \eqref{eq:dfdivide} and
    the lower bound on $h$ and \eqref{eq:vDiff}
    and \eqref{eq:Nofdeltadef_nlin}
    we can write the following estimates:

    \begin{gather*}
        h^{-\theta}
        \enbrace{\frac{h_0}{2\Cbdistort}}^{\theta-1}
        \vmod{ \hat{S}_{N} } =
        h^{1-\theta}
        \enbrace{\frac{h_0}{2\Cbdistort}}^{\theta-1}
        \vmod{
            \sum_{i=0}^{N} v'(f^i(x))
            \frac{ \dfxoth{i}{x}   }{\dfxthxp{f^i(x) }} 
        } \leq 
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \\ \leq
        \vmod{ \sum_{i=0}^{N} v'(f^i(x))
        \frac{ \dfxoth{i}{x} }
        { \dfxthxp{f^i(x)} \dfxoth{N_h}{x} }
    } \leq 
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \\ \leq
        \frac{1 }{\lambda^{\theta}}
        \vmod{ 
            \sum_{i=0}^{N} v'(f^i(x))
        \frac{ 1 }{  \dfxoth{N_h-i}{f^{i}(x)  } } } \leq 
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \\ \leq  
            \frac{\maxvprime }{\lambda^{\theta}}
            \enbrace{  
                 \sum_{i = 0}^{N}
                \lambda^{ -(N_h-i) (1- \theta) }   }
                \leq 
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                \\ \leq 
                    \frac{2\maxvprime
                        \lambda^{-(N_h-N)(1-\theta)-\theta}
             } {1 -\lambda^{ -1+\theta } }
             \leq
                    \frac{4\maxvprime
                        }
                     { \lambda^{(N_h-N)(1-\theta)+\theta } }
            \end{gather*}
        \end{proof}

        {\bfseries 
            [Note that here we used that $\theta<1$. Otherwise the
                estimate for the sum $\sum_0^{N} \lambda^{(N_h-i)(1-\theta) = N}$
            is not useful]
        }


==> upper_bound_lin.tex <==
\begin{lm} \label{lm:lin_upper_bd}

    Let $N$ be a natural number,  $h_0>0$
    and $h>0$ be such that
    \begin{gather*}  %\label{eq:Ndef_lin_lm}
       %\frac{1}{ \dfxth{N} }  
        \frac{ h_0}{ 2\lambda^{N} } \leq h \leq
        \frac{ h_0 }{ \lambda^{N} }  
        .
    \end{gather*}

    %\input{hcond_lin}
    Then %for every natural $N$
    \begin{gather*}
        h^{-\theta} \vmod{ \hat{S}_{N} }    % \label{neq:ubound_lin}
        \leq
                4\frac{\maxvprime}{\lambda^{(N_h-N)(1-\theta) + \theta}}
        h_0^{1-\theta}
    \end{gather*}
\end{lm}

\begin{proof}
        Note that 
    \begin{gather*}
        h^{1-\theta} h_0^{-1+\theta} \frac{\lambda^i}{\lambda^{(i+1)\theta} } 
        \leq \lambda^{-(N_h-i)(1-\theta) - \theta}
    \end{gather*}

    Then using the upper bound for $h$ 
    we can write the following estimates:
    \begin{gather*}
        h^{-\theta}
        h_0^{-1+\theta}
        \vmod{ \hat{S}_{N} } =
        h^{1-\theta} 
        h_0^{-1+\theta}
        \vmod{
            \sum_{i=0}^{N} v'(f^i(x))
            \frac{ \lambda^{i}   }{\lambda^{(i+1)\theta} } 
        } \leq 
        \\
        \leq
        \frac{1}{\lambda^{\theta}} 
            \vmod{
                 \sum_{i=0}^{N} v'(f^i(x))
            \frac{  1 }
            {  \lambda^{(N_h-i)(1-\theta)}  } }    
            \leq 
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \\
            \leq  
            \frac{\maxvprime}{\lambda^{\theta}}
                 \sum_{i = 0}^{N}
                \lambda^{ -(N_h-i) (1- \theta) }  
                \leq 
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                \\ \leq 
                \frac{\maxvprime}{\lambda^{(N_h-N)(1-\theta) + \theta}}
                 \frac{2 } {1 -\lambda^{ -1+\theta } }  
                 \leq      % use big lambda
                4\frac{\maxvprime}{\lambda^{(N_h-N)(1-\theta) + \theta}}
                    .
            \end{gather*}

        \end{proof}

